MoxE: Mixture of xLSTM Experts with Entropy-Aware Routing for Efficient Language Modeling

This paper introduces MoxE, a novel architecture that synergistically combines the Extended Long Short-Term Memory (xLSTM) with the Mixture of Experts (MoE) framework to address critical scalability and efficiency challenges in large language models (LLMs). The proposed method effectively leverages xLSTM's innovative memory structures while strategically introducing sparsity through MoE to substantially reduce computational overhead. At the heart of our approach is a novel entropy-based routing mechanism, designed to dynamically route tokens to specialized experts, thereby ensuring efficient and balanced resource utilization. This entropy awareness enables the architecture to effectively manage both rare and common tokens, with mLSTM blocks being favored to handle rare tokens. To further enhance generalization, we introduce a suite of auxiliary losses, including entropy-based and group-wise balancing losses, ensuring robust performance and efficient training. Theoretical analysis and empirical evaluations rigorously demonstrate that MoxE achieves significant efficiency gains and enhanced effectiveness compared to existing approaches, marking a notable advancement in scalable LLM architectures.

==> methodology_figure.tex <==

\begin{tikzpicture}[
    font=\small,
    >=Stealth,
    line/.style={->, thick},
    box/.style={draw, rounded corners, align=center, minimum width=2.6cm, minimum height=1.0cm},
    bigbox/.style={draw, thick, rounded corners, inner sep=0.3cm},
    dashedbox/.style={draw, dashed, rounded corners},
    every node/.style={font=\small},
    fire/.style={text=red!70!orange, font=\faFire},
    ice/.style={text=cyan!80!blue, font=\faSnowflake},
    circle_op/.style={circle, draw, minimum size=0.8cm, text centered, font=\Large, thick}, % Added thick
]
    %% ------------------------------------------------
    %% 1) Top-level: Input token
    %% ------------------------------------------------
    \node[box, fill=gray!20] (inputtoken) {Input Sequence};
    
    %% ------------------------------------------------
    %% 2) Student pipeline (left) -- blue palette
    %% ------------------------------------------------
    \node[box, fill=yellow!20, below left=1.5cm and 1.5cm of inputtoken] (studemb) {Embeddings \hspace{0.2em} \small{\textcolor{cyan!80!blue}{\faSnowflake}}};
    \node[box, fill=yellow!30, below=1.2cm of studemb] (xlstm) {xLSTM blocks \hspace{0.2em} \small{\textcolor{red!70!orange}{\faFire}}};
    \node[box, fill=yellow!40, below=1.5cm of xlstm] (lmhead_stud) {LM Head \hspace{0.2em} \small{\textcolor{cyan!80!blue}{\faSnowflake}}};
    \node[box, fill=yellow!10, below=1cm of lmhead_stud] (studlogits) {Student logits};
    
    % Bounding box around Student portion
    \node[bigbox, label={[yellow!60!black]above:Student}, fit=(studemb)(xlstm)(lmhead_stud)] (studentbox) {};
    
    % Connect Student pipeline
    \draw[line] (inputtoken) to[out=180, in=0] (studemb);
    \draw[line] (studemb) -- (xlstm);
    \draw[line] (xlstm) -- (lmhead_stud);
    \draw[line] (lmhead_stud) -- (studlogits);
    
    %% ------------------------------------------------
    %% 3) Teacher pipeline (right) -- orange palette
    %% ------------------------------------------------
    \node[box, fill=orange!20, below right=1.5cm and 1.5cm of inputtoken] (teachemb) {Embeddings \hspace{0.2em} \small{\textcolor{cyan!80!blue}{\faSnowflake}}};
    \node[box, fill=orange!30, below=1.2cm of teachemb] (attn) {Attention blocks \hspace{0.2em} \small{\textcolor{red!70!orange}{\faFire}}};
    \node[box, fill=orange!40, below=1.5cm of attn] (lmhead_teach) {LM Head \hspace{0.2em} \small{\textcolor{cyan!80!blue}{\faSnowflake}}};
    \node[box, fill=orange!10, below=1cm of lmhead_teach] (teachlogits) {Teacher logits};
    
    % Bounding box around Teacher portion
    \node[bigbox, label={[orange!70!black]above:Teacher}, fit=(teachemb)(attn)(lmhead_teach)] (teacherbox) {};
    
    % "Mixer" sections with contrasting dashed borders
    \node[draw, dashed, blue!70, thick, fit=(xlstm) (attn), inner sep=15pt] (sequence_mixer) {Sequence Mixer};
    \node[draw, dashed, teal!70!black, thick, fit=(lmhead_stud) (lmhead_teach), inner sep=15pt] (channel_mixer) {Channel Mixer};
    
    % Connect Teacher pipeline
    \draw[line] (inputtoken) to[out=0, in=180] (teachemb);
    \draw[line] (teachemb) -- (attn);
    \draw[line] (attn) -- (lmhead_teach);
    \draw[line] (lmhead_teach) -- (teachlogits);
    
    %% ------------------------------------------------
    %% 4) Outputs, losses, etc.
    %% ------------------------------------------------
    \node[box, fill=purple!20, below=1.0cm of studlogits] (task_loss) {$\mathcal{L}_{CE}$};
    \node[box, fill=gray!20, left=1.0cm of studlogits] (hardlabels) {Hard labels};
    \node[box, fill=red!20, below=1.0cm of teachlogits] (klblock) {$\mathcal{L}_{KD}$};
    \node[box, fill=red!30, below=1.8cm of $(task_loss)!0.5!(klblock)$] (total_loss) {Total loss};

    % Summation node
    \node[circle_op] (sum) at ($(task_loss.east)!0.5!(klblock.west)$) {$\Sigma$};
    
    % Connect outputs
    \draw[line] (hardlabels) to[out=270, in=180] (task_loss);
    \draw[line] (studlogits) -- (task_loss);
    \draw[line] (task_loss) -- (sum);
    \draw[line] (studlogits) to[out=0, in=140] (klblock);
    \draw[line] (teachlogits) -- (klblock);
    \draw[line] (klblock) -- (sum);
    \draw[line] (sum) -- (total_loss);
    
    %% ------------------------------------------------
    %% 5) Legend
    %% ------------------------------------------------
    \node[below=1.0cm of total_loss, xshift=-2cm] (frozen_legend) {\textcolor{cyan!80!blue}{\faSnowflake} Frozen parameters};
    \node[below=1.0cm of total_loss, xshift=2cm] (trainable_legend) {\textcolor{red!70!orange}{\faFire} Trainable parameters};
\end{tikzpicture}

